Deep Learning Analysis of Deeply Virtual Exclusive Photoproduction

We present a Machine Learning based approach to the cross section and asymmetries for deeply virtual Compton scattering from an unpolarized proton target using both an unpolarized and polarized electron beam. Machine learning methods are needed to study and eventually interpret the outcome of deeply virtual exclusive experiments since these reactions are characterized by a complex final state with a larger number of kinematic variables and observables, exponentially increasing the difficulty of quantitative analyses. Our deep neural network (FemtoNet) uncovers emergent features in the data and learns an accurate approximation of the cross section that outperforms standard baselines. FemtoNet reveals that the predictions in the unpolarized case systematically show a smaller relative median error than the polarized that can be ascribed to the presence of the Bethe Heitler process. It also suggests that the $t$ dependence can be more easily extrapolated than for the other variables, namely the skewness, $\xi$ and four-momentum transfer, $Q^2$. Our approach is fully scalable and will be capable of handling larger data sets as they are released from future experiments.

==> sections/inference/results.tex <==
\subsection{Comparing FemtoNet Results to Baselines and Theory}

==> sections/inference/uncertainty-plots.tex <==
\subsection{Model Uncertainty across Kinematic Space}
\begin{center}
\begin{figure}[h]
\includegraphics[scale=0.4]{figures/2d_median_absolute_percentage_error.png}
\caption{Mean absolute percentage discrepancy as a function of kinematic variables $\xi$ and $t$ comparing neural network predictions to theoretical predictions of the cross section for the unpolarized cross section at $Q^{2} = 2 \,\, \text{GeV}^{2}$ and $\text{E}_{b} = 5.75 \,\, \text{GeV}$.}
\end{figure}
\end{center}

